BMRS: Bayesian Model Reduction for Structured Pruning

Modern neural networks are often massively overparameterized leading to high compute costs during training and at inference. One effective method to improve both the compute and energy efficiency of neural networks while maintaining good performance is structured pruning, where full network structures (e.g.~neurons or convolutional filters) that have limited impact on the model output are removed. In this work, we propose Bayesian Model Reduction for Structured pruning (BMRS), a fully end-to-end Bayesian method of structured pruning. BMRS is based on two recent methods: Bayesian structured pruning with multiplicative noise, and Bayesian model reduction (BMR), a method which allows efficient comparison of Bayesian models under a change in prior. We present two realizations of BMRS derived from different priors which yield different structured pruning characteristics: 1) BMRS_N with the truncated log-normal prior, which offers reliable compression rates and accuracy without the need for tuning any thresholds and 2) BMRS_U with the truncated log-uniform prior that can achieve more aggressive compression based on the boundaries of truncation. Overall, we find that BMRS offers a theoretically grounded approach to structured pruning of neural networks yielding both high compression rates and accuracy. Experiments on multiple datasets and neural networks of varying complexity showed that the two BMRS methods offer a competitive performance-efficiency trade-off compared to other pruning methods.

==> neurips_rebuttal/runtimes.tex <==

% \begin{table}%[htp]
%     %\setlength{\tabcolsep}{1.5pt}
%     \def\arraystretch{1.2}
%     \centering
%     %\fontsize{10}{10}\selectfont
%     \scriptsize
%     %\rowcolors{2}{gray!10}{white}
%     \begin{tabular}{l | c | c | c | c}
%     \toprule %\thickhline
%     \multicolumn{1}{c}{ Pruning Method } & \multicolumn{1}{c}{ MNIST } & \multicolumn{1}{c}{Fash-MNIST} & \multicolumn{1}{c}{CIFAR10} & \multicolumn{1}{c}{TinyImagenet} \\

% \midrule
% \multicolumn{5}{c}{MLP}\\
% \midrule
% None & 00h02m00s & 00h04m07s & 00h12m55s & -\\
% SNR & 00h09m47s & 00h03m13s & 00h25m14s & -\\
% BMRS & 00h12m13s & 00h03m47s & 00h28m38s & \\

% \midrule
% \multicolumn{5}{c}{Lenet5}\\
% \midrule
% None & 00h01m54s & 00h04m19s & 00h07m21s & - \\
% SNR & 00h09m41s & 00h20m07s & 00h12m46s & -\\
% BMRS & 00h03m47s & 00h13m50s & 00h11m12s & - \\

% \midrule
% \multicolumn{5}{c}{Resnet50}\\
% \midrule
% None & - & - & 05h38m48s & 11h59m00s\\
% SNR & - & - & 26h18m25s & 56h24m42s \\
% BMRS & & & & 56h44m03s \\

% \midrule
% \multicolumn{5}{c}{ViT}\\
% \midrule
% None & - & - & 27h18m42s & 30h00m40s \\
% SNR & - & - & 33h01m55s & 42h52m33s \\
% BMRS & - & - & 21h30m28s & 42h42m48s \\


%     \bottomrule % \thickhline

%     \end{tabular}
%     \caption{Parameter compression \% and accuracy. Results are averaged across 10 runs. Standard deviation given in subscript.} %Results are reported as the average macro F1 over 5 random seeds.}
%     \label{tab:small_results}
% \end{table}

\begin{table}%[htp]
    %\setlength{\tabcolsep}{1.5pt}
    \def\arraystretch{1.2}
    \centering
    %\fontsize{10}{10}\selectfont
    % \scriptsize
    \footnotesize
    %\rowcolors{2}{gray!10}{white}
    \begin{tabular}{l  c  c  c | c  c }
    \toprule %\thickhline
    \multicolumn{1}{c}{ \multirow{2}{*}{Pruning Method} } &
    \multicolumn{3}{c|}{Lenet5} & 
    \multicolumn{2}{c}{ViT} \\
\cmidrule{2-4} 
\cmidrule{5-6}
    & \multicolumn{1}{c}{ MNIST } & \multicolumn{1}{c}{Fash-MNIST} & \multicolumn{1}{c|}{CIFAR10} & 
    \multicolumn{1}{c}{TinyImagenet} &
    \multicolumn{1}{c}{CIFAR10} 
   \\ 
    % \multicolumn{1}{c}{TinyImagenet} \\

% \multicolumn{5}{c}{Lenet5}\\
\midrule
None & 00h01m54s & 00h04m19s & 00h07m21s & 30h00m40s &  27h18m42s\\
SNR & 00h09m41s & 00h20m07s & 00h12m46s & 42h52m33s & 33h01m55s\\
BMRS & 00h06m17s & 00h22m52s & 00h14m52s & 42h42m48s & 21h30m28s\\

% \midrule
% \multicolumn{5}{c}{ViT}\\
% \midrule
% None & - & - & 27h18m42s & 30h00m40s \\
% SNR & - & - & 33h01m55s & 42h52m33s \\
% BMRS & - & - & 21h30m28s & 42h42m48s \\


    \bottomrule % \thickhline

    \end{tabular}
    \caption{Full training runtimes for Lenet5 and ViT.} %Results are reported as the average macro F1 over 5 random seeds.}
    \label{tab:small_results}
\end{table}


==> neurips_rebuttal/table1.tex <==

\begin{table}%[htp]
    %\setlength{\tabcolsep}{1.5pt}
    \def\arraystretch{1.2}
    \centering
    %\fontsize{10}{10}\selectfont
    %\scriptsize
    \footnotesize       
    %\rowcolors{2}{gray!10}{white}
    \begin{tabular}{l c c | c c | c c}
    \toprule %\thickhline
    & \multicolumn{2}{c}{ MNIST } & \multicolumn{2}{c}{ Fash-MNIST } & \multicolumn{2}{c}{ CIFAR10 } \\
    \midrule
    Pruning Method & Comp \% & Acc. & Comp \% & Acc. & Comp \% & Acc.\\

\midrule
\multicolumn{7}{c}{MLP}\\
\midrule
None&$0.00 \pm 0.00$& $97.43 \pm 0.14$& $0.00 \pm 0.00$& $88.17 \pm 0.20$& $0.00 \pm 0.00$& $44.94 \pm 0.40$\\
L2&$43.11 \pm 2.06$& $10.39 \pm 0.32$& $87.86 \pm 2.27$& $18.23 \pm 10.22$& $42.89 \pm 2.64$& $10.00 \pm 0.00$\\
\rowcolor{yellow}$E[\theta]$&$52.08 \pm 1.71$& $96.88 \pm 0.15$& $91.76 \pm 0.81$& $85.59 \pm 0.26$& $77.99 \pm 1.54$& $43.39 \pm 0.46$ \\
SNR&$58.57 \pm 2.01$& $96.92 \pm 0.08$& $99.83 \pm 0.00$& $10.00 \pm 0.00$& $75.93 \pm 1.26$& $43.97 \pm 0.46$\\
\methodn{}&$48.86 \pm 1.32$& $96.95 \pm 0.19$& $93.20 \pm 0.66$& $84.99 \pm 0.35$& $76.36 \pm 1.08$& $43.59 \pm 0.29$\\
\methodu{}-8&$48.73 \pm 1.90$& $96.93 \pm 0.16$& $93.02 \pm 0.81$& $85.01 \pm 0.32$& $77.17 \pm 0.98$& $43.45 \pm 0.42$\\
\methodu{}-4&$54.47 \pm 1.74$& $\mathbf{96.99 \pm 0.13}$& $91.57 \pm 0.71$& $\mathbf{85.79 \pm 0.34}$& $76.63 \pm 0.94$& $\mathbf{44.06 \pm 0.40}$\\
\midrule
\multicolumn{7}{c}{Lenet5}\\
\midrule
None&$0.00 \pm 0.00$& $99.07 \pm 0.09$& $0.00 \pm 0.00$& $89.16 \pm 0.27$& $0.00 \pm 0.00$& $67.62 \pm 0.77$\\
L2&$83.42 \pm 1.92$& $11.35 \pm 0.00$& $83.62 \pm 1.69$& $10.00 \pm 0.00$& $52.29 \pm 2.18$& $10.00 \pm 0.00$\\
\rowcolor{yellow}$E[\theta]$&$88.29 \pm 1.00$& $51.30 \pm 41.12$& $89.71 \pm 0.56$& $50.93 \pm 33.45$& $66.19 \pm 1.36$& $65.83 \pm 0.90$\\
SNR&$92.66 \pm 5.77$& $62.70 \pm 41.93$& $98.47 \pm 3.45$& $17.01 \pm 21.03$& $70.29 \pm 2.02$& $\mathbf{67.68 \pm 0.52}$\\
\methodn{}&$86.90 \pm 1.15$& $95.59 \pm 0.94$& $88.02 \pm 1.00$& $77.90 \pm 2.44$& $62.87 \pm 1.64$& $66.14 \pm 0.70$\\
\methodu{}-8&$86.11 \pm 1.37$& $95.27 \pm 1.02$& $87.61 \pm 0.72$& $77.23 \pm 3.49$& $62.54 \pm 1.49$& $66.28 \pm 1.07$\\
\methodu{}-4&$87.58 \pm 1.01$& $\mathbf{96.66 \pm 0.59}$& $88.72 \pm 0.73$& $\mathbf{81.10 \pm 1.50}$& $68.07 \pm 1.95$& $67.66 \pm 0.59$\\

    \bottomrule % \thickhline

    \end{tabular}
    \caption{Average parameter compression \% and accuracy ($\pm$ standard deviation).} %Results are reported as the average macro F1 over 5 random seeds.}
    \label{tab:small_results}
\end{table}


==> tables/metrics.tex <==

\begin{table}%[htp]
    %\setlength{\tabcolsep}{1.5pt}
    \def\arraystretch{1.2}
    \centering
    \fontsize{10}{10}\selectfont
    \rowcolors{2}{gray!10}{white}
        \caption{Neuron compression \% and accuracy. Results are averaged across 10 runs. Standard deviation given in subscript.} %Results are reported as the average macro F1 over 5 random seeds.}
    \label{tab:{dataset}_results}
    \begin{tabular}{l c c | c c | c c}
    \toprule %\thickhline
    & \multicolumn{2}{c}{ MNIST } & \multicolumn{2}{c}{ Fash-MNIST } & \multicolumn{2}{c}{ CIFAR10 } \\
    \midrule
    Pruning Method & Comp \% & Acc. & Comp \% & Acc. & Comp \% & Acc.\\

\midrule
\multicolumn{7}{c}{MLP}\\
\midrule
None&$0.00_{0.00}$& $97.43_{0.14}$& $0.00_{0.00}$& $88.17_{0.20}$& $0.00_{0.00}$& $44.94_{0.40}$\\
SNR&$81.31_{0.81}$& $96.97_{0.25}$& $100.00_{0.00}$& $10.00_{0.00}$& $88.03_{0.60}$& $43.97_{0.46}$\\
Approximate Spike&$68.34_{1.82}$& $96.95_{0.15}$& $81.47_{9.84}$& $84.93_{0.31}$& $88.19_{0.38}$& $43.70_{0.28}$\\
CDF&$80.69_{1.03}$& $96.94_{0.19}$& $91.70_{0.41}$& $85.86_{0.24}$& $88.09_{0.58}$& $43.87_{0.17}$\\
\midrule
\multicolumn{7}{c}{Lenet5}\\
\midrule
None&$0.00_{0.00}$& $99.07_{0.09}$& $0.00_{0.00}$& $89.16_{0.27}$& $0.00_{0.00}$& $67.62_{0.77}$\\
SNR&$90.50_{7.78}$& $62.75_{41.97}$& $98.68_{3.96}$& $17.01_{21.03}$& $70.71_{1.64}$& $67.68_{0.52}$\\
Approximate Spike&$45.85_{2.41}$& $94.58_{0.91}$& $51.88_{2.19}$& $74.70_{3.49}$& $38.90_{1.36}$& $66.61_{0.89}$\\
CDF&$90.31_{6.38}$& $71.17_{39.16}$& $88.89_{3.76}$& $73.99_{21.35}$& $72.94_{1.60}$& $67.78_{0.51}$\\
\midrule
\multicolumn{7}{c}{Res50}\\
\midrule
None&$-$& $-$& $-$& $-$& $0.00_{0.00}$& $84.53_{0.13}$\\
SNR&$-$& $-$& $-$& $-$& $76.32_{0.98}$& $84.02_{0.16}$\\
Approximate Spike&$-$& $-$& $-$& $-$& $60.10_{6.46}$& $82.68_{0.77}$\\
CDF&$-$& $-$& $-$& $-$& $-$& $-$\\
\midrule
\multicolumn{7}{c}{Res50-Pretrained}\\
\midrule
None&$-$& $-$& $-$& $-$& $0.00_{0.00}$& $90.67_{0.05}$\\
SNR&$-$& $-$& $-$& $-$& $84.94_{0.11}$& $89.53_{0.02}$\\
Approximate Spike&$-$& $-$& $-$& $-$& $76.52_{2.29}$& $89.74_{0.41}$\\
CDF&$-$& $-$& $-$& $-$& $-$& $-$\\
\midrule
\multicolumn{7}{c}{Vision Transformer}\\
\midrule
None&$-$& $-$& $-$& $-$& $0.00_{0.00}$& $95.03_{0.00}$\\
SNR&$-$& $-$& $-$& $-$& $89.11_{0.00}$& $94.92_{0.00}$\\
Approximate Spike&$-$& $-$& $-$& $-$& $70.37_{0.31}$& $94.60_{0.01}$\\
CDF&$-$& $-$& $-$& $-$& $-$& $-$\\

    \bottomrule % \thickhline

    \end{tabular}
\end{table}

